SU(N) fractional Instantons

We present our study of a set of solutions to the $SU(N)$ Yang-Mills equations of motion with fractional topological charge. The configurations are obtained numerically by minimizing the action with gradient flow techniques on a torus of size $l^2\times(Nl)^2$ with twisted boundary conditions. We pay special attention to the large $N$ limit, which is taken along a very peculiar sequence, with the number of colors $N$ and the magnetic flux $m$ selected respectively as the $n$-th and $n-2$ terms of the Fibonacci sequence. We discuss the large $N$ scaling of the solutions and analyze several gauge invariant quantities as the Polyakov loops. We also discuss the so-called Hamiltonian limit, with one of the large directions sent to infinity, where these instantons represent tunneling events between inequivalent pure gauge configurations.

==> flat.tex <==
%\section{Constant curvature solutions on $ \mathbf T^4$}
%\label{sec:flat}
%\input{flat.tex}

Our selection of twist parameters within the Fibonacci sequence is suitable for easily constructing self-dual solutions to the YM equation with fractional topological charge $Q=1/N$. This is based in the construction presented in ref. \cite{Gonzalez-Arroyo:2019wpu}. The Hamiltonian limit discussed in the introduction is not included in this construction, but the comparison with it is very clarifying, as goes on the line exposed in ref. \cite{Gonzalez-Arroyo:2019wpu,GarciaPerez:2000aiw} of interpreting this solutions as deformations of this constant curvature construction. 

\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\linewidth]{plots/L_L2NL2_kk_plana1.pdf}
\caption{Several solutions for different values of time extent $l_0$. }
\label{fig:flat}
\end{figure}

The complete deduction can be found in ref. \cite{DasilvaGolan:2022jlm}. The important result is that taking $m=F_{n-2}$ and $N=F_{n}$, self-dual solutions to the YM equations exist for any value of $l_0$ satisfying:
\be
l_0 l_3= \frac{F_{n-m+1} F_{n-m}} {F_n^2 F_{m} F_{m-1}} 
\label{eq:fibonacci-cc}
\ee
where we have scaled $l_1=l_2=1/F_n$. 

We have generated several numerical simulations starting at $l_0=0.25l$ (very close to the Fibonacci case), and growing up to $l_0=1.00l$. The energy density profile is shown if figure~\ref{fig:flat}. The solutions change rapidly at the beginning, but beyond $l_0\sim0.5 l$ it remains unchanged except at the tails where it decays exponentially.

